Versatile Verification of Tree Ensembles

Machine learned models often must abide by certain requirements (e.g., fairness or legal). This has spurred interested in developing approaches that can provably verify whether a model satisfies certain properties. This paper introduces a generic algorithm called Veritas that enables tackling multiple different verification tasks for tree ensemble models like random forests (RFs) and gradient boosting decision trees (GBDTs). This generality contrasts with previous work, which has focused exclusively on either adversarial example generation or robustness checking. Veritas formulates the verification task as a generic optimization problem and introduces a novel search space representation. Veritas offers two key advantages. First, it provides anytime lower and upper bounds when the optimization problem cannot be solved exactly. In contrast, many existing methods have focused on exact solutions and are thus limited by the verification problem being NP-complete. Second, Veritas produces full (bounded suboptimal) solutions that can be used to generate concrete examples. We experimentally show that Veritas outperforms the previous state of the art by (a) generating exact solutions more frequently, (b) producing tighter bounds when (a) is not possible, and (c) offering orders of magnitude speed ups. Subsequently, Veritas enables tackling more and larger real-world verification scenarios.

==> problem.tex <==
% vim: filetype=tex

\section{High-Level Problem Description}

We formally define the generic optimization problem that is used to solve the verification tasks.
Consider predictive models $\bm{T}_1$ and $\bm{T}_2$ which produce outputs $\bm{T}_1(\bm{x}_1)$ and $\bm{T}_2(\bm{x}_2)$ for data examples $\bm{x}_1$ and $\bm{x}_2$ from the input space $\mathcal{X}$.
Let $\mathcal{C} : \mathcal{X}^2 \rightarrow \{\mathrm{true}, \mathrm{false}\}$ be a function defining constraints on the input spaces of the models.
The optimization problem is then defined as:
\begin{equation}
    \label{eq:opt2}
    \max_{
        \bm{x}_1, \bm{x}_2 \in \mathcal{X}
    } \bm{T}_2(\bm{x}_2)  - \bm{T}_1(\bm{x}_1)
    \quad \text{subject to}
    \quad \mathcal{C}(\bm{x}_1, \bm{x}_2).
\end{equation}
In words: \textit{find two data examples that satisfy the constraints and that maximize the difference between the outputs of the two models}.

In many cases, we only consider a single model $\bm{T}$. By taking $\bm{T}_1$ to be the trivial model that always predicts 0.0, and $\bm{T}_2 = \bm{T}$, we solve the following optimization problem:
\begin{equation}
    \label{eq:opt1}
    \max_{\bm{x}\in\mathcal{X}} \bm{T}(\bm{x}) 
    \quad \text{subject to}
    \quad \mathcal{C}(\bm{x}).
\end{equation}
Minimizing $\bm{T}$ is also possible by taking $\bm{T}_1 = \bm{T}$, and making $\bm{T}_2$ the trivial model. Note that we simplify $\mathcal{C}$ because the example of the trivial model does not affect the outcome.

To see why these optimization problems are useful, consider the following examples:
\begin{itemize}
    \item Assume $\bm{T}$ to be a binary classifier.
        We can check whether $\bm{T}$ is $\delta$-robust with respect to an example $\hat{\bm{x}}$ as follows. Assume $\hat{\bm{x}}$ has the negative class, i.e., $\bm{T}(\hat{\bm{x}}) < 0$. Let $\mathcal{C} : \bm{x} \mapsto {|| \bm{x} - \hat{\bm{x}} ||}_\infty < \delta$ accept only the data examples that lie within a $\delta$ distance from $\hat{\bm{x}}$.
        If the value $\bm{T}(\bm{x}^*)$ returned by the optimization procedure is greater than 0, then the model is not $\delta$-robust for $\hat{\bm{x}}$. The generated data example $\bm{x}^*$ is an adversarial example. In the other case, we say $\bm{T}$ is $\delta$-robust with respect to $\hat{\bm{x}}$.
    \item Assume an insurance company uses model $\bm{T}$ to estimate a health score of a client. Assume the company wants to know which attributes affect the health score of middle-aged Caucasian women the most. Pick one attribute and let $\mathcal{C}$ only accept pairs of examples that differ in that attribute and belong to the target group. Then, compute the maximum output difference. Repeat this process for each attribute of interest. The attribute with the highest output difference is the most dominant.
\end{itemize}
Previous work has established that the verification problem of tree ensembles -- the models we will consider -- is NP-complete \cite{kantchelian16}, so it is expected that many problems cannot be solved exactly. In that case, we wish the output of Equation~\ref{eq:opt2} to be upper and lower bounds $\bar{b}$ and $\ubar{b}$, and a bounded suboptimal full solution $\tilde{\bm{x}}$, $\ubar{b} \leq \bm{T}(\tilde{\bm{x}}) \leq \bar{b}$.

%Let $\bm{T}$ be a tree ensemble model which produces an output $\bm{T}(\bm{x})$ for a data example $\bm{x}$ from the input space $\mathcal{X}$. Consider function $\mathcal{C} : \mathcal{X} \rightarrow \{\mathrm{true}, \mathrm{false}\}$ defining constraints on the input space $\mathcal{X}$. The optimization problem solved in this paper is defined as follows:
%\begin{equation}
%    \label{eq:opt1}
%    \max_{\bm{x}\in\mathcal{X}} \bm{T}(\bm{x}) 
%    \quad \text{subject to}
%    \quad \mathcal{C}(\bm{x})\ \text{is}\ \mathrm{true}.
%\end{equation}
%In words, Equation~\ref{eq:opt1} expresses: find the data instance $\bm{x}$ that adheres to the constraints defined by $\mathcal{C}$ and maximizes the model output $\bm{T}(\bm{x})$. Let $\bm{x}^*$ be the unknown optimal solution. Our proposed algorithm will produce lower and upper bounds $\ubar{b}$ and $\bar{b}$ such that $\ubar{b} \leq \bm{T}(\bm{x}^*) \leq \bar{b}$.
%For the lower bound $\ubar{b}$, an accompanying full solution $\ubar{\bm{x}} \in \mathcal{X}$ is generated such that $\bm{T}(\ubar{\bm{x}}) = \ubar{b}$. This solution is useful in many cases, as will become clear in the experiments. \ld{check}
%
%The task in Equation~\ref{eq:opt1} can be further generalized to the problem of maximizing the difference between two ensemble models $\bm{T}_1$ and $\bm{T}_2$. The models have input spaces $\mathcal{X}_1$ and $\mathcal{X}_2$, and the constraint function $\mathcal{C}$ accepts or rejects pairs of data instances $(\bm{x}_1, \bm{x}_2)$, one for each model:
%\begin{equation}
%    \label{eq:opt2}
%    \max_{
%        \begin{subarray}{l}
%            \bm{x}_1\in\mathcal{X}_1, \\
%            \bm{x}_2\in\mathcal{X}_2
%        \end{subarray}
%    } \bm{T}_2(\bm{x}_2)  - \bm{T}_1(\bm{x}_1)
%    \ \text{subject to}
%    \ \mathcal{C}(\bm{x}_1, \bm{x}_2)\ \text{is}\ \mathrm{true}.
%\end{equation}
%Depending on the verification task, it is possible to have $\bm{x}_1 = \bm{x}_2$ or $\bm{T}_1 = \bm{T}_2$. In this setting, $\mathcal{C}$ can restrict both input spaces, but also define constraints between the two instances $\bm{x}_1$ and $\bm{x}_2$. As before, our method generates $\ubar{b}$ and $\bar{b}$, lower and upper bounds on the difference between the outputs of the two models, and $\ubar{\bm{x}}_1$ and $\ubar{\bm{x}}_2$.
%
%Note that the task in Equation~\ref{eq:opt2} encompasses the task in Equation~\ref{eq:opt1}. For maximization, take $\bm{T}_1$ to be the trivial model that always predicts zero, then $\bm{T}_2$ is maximized. If $\bm{T}_2$ is taken to be the trivial model, then $\bm{T}_1$ is minimized.

